Low-variance estimation in the Plackett-Luce model via quasi-Monte Carlo sampling

The Plackett-Luce (PL) model is ubiquitous in learning-to-rank (LTR) because it provides a useful and intuitive probabilistic model for sampling ranked lists. Counterfactual offline evaluation and optimization of ranking metrics are pivotal for using LTR methods in production. When adopting the PL model as a ranking policy, both tasks require the computation of expectations with respect to the model. These are usually approximated via Monte-Carlo (MC) sampling, since the combinatorial scaling in the number of items to be ranked makes their analytical computation intractable. Despite recent advances in improving the computational efficiency of the sampling process via the Gumbel top-k trick, the MC estimates can suffer from high variance. We develop a novel approach to producing more sample-efficient estimators of expectations in the PL model by combining the Gumbel top-k trick with quasi-Monte Carlo (QMC) sampling, a well-established technique for variance reduction. We illustrate our findings both theoretically and empirically using real-world recommendation data from Amazon Music and the Yahoo learning-to-rank challenge.

==> listings/Makefile <==
### Makefile ---
#
# This file generates files required to use the listings package.
#
# $Id$
#
# (c) 2007 Brooks Moses
# (c) 2013-2018 Jobst Hoffmann
#
# This file is distributed under the terms of the LaTeX Project Public
# License from CTAN archives in directory  macros/latex/base/lppl.txt.
# Either version 1.3c or, at your option, any later version.

# remember:
# $<: first element of list of dependees
# $^: list of (all) dependees
# $@: target

# formatting tools
LATEX = pdflatex
MAKEINDEX = makeindex
TEX = tex
# tarring options
ifneq "$(wildcard listings.version)" ""
include listings.version        # version and date of the package
endif
TAR_SRC = $(PACKAGE)-$(VERSION)_source.tgz
EXsvn = --exclude .svn --exclude auto --exclude contrib --exclude requests \
	--exclude support --exclude testing \
	--exclude *.tgz --exclude *.txt

DISTRIBUTION_FILES = ../$(PACKAGE)/$(PACKAGE).pdf \
	../$(PACKAGE)/$(PACKAGE)-devel.pdf \
	../$(PACKAGE)/$(PACKAGE).dtx \
	../$(PACKAGE)/$(PACKAGE).ins \
	../$(PACKAGE)/README \
	../$(PACKAGE)/Makefile \
	../$(PACKAGE)/lstdrvrs.dtx \
	../$(PACKAGE)/lstdrvrs.pdf 
PACKAGE_FILES = $(subst ../$(PACKAGE)/,,$(DISTRIBUTION_FILES))
STY_FILES = listings.cfg listings.sty lstmisc.sty \
	lstlang0.sty lstlang1.sty lstlang2.sty

.SUFFIXES:                              # Delete the default suffixes
.SUFFIXES: .dtx .ins .pdf .sty          # Define our own suffix list

.PHONY: listings pdf pdf-devel tests all

listings: listings.sty

pdf: listings.pdf lstdrvrs.pdf

pdf-devel: listings-devel.pdf

all: listings pdf pdf-devel


listings.sty: listings.ins listings.dtx lstdrvrs.dtx
	$(TEX) $<

listings.pdf: listings.sty
	echo "\PassOptionsToClass{a4paper}{article}" > ltxdoc.cfg
	$(LATEX) ${<:.sty=.dtx}
	$(MAKEINDEX) -s gind.ist ${@:.pdf=}
	$(LATEX) ${<:.sty=.dtx}
	$(LATEX) ${<:.sty=.dtx}
	rm -f ltxdoc.cfg

listings-devel.pdf: listings.sty
	echo "\PassOptionsToClass{a4paper}{article}" > ltxdoc.cfg
	echo "\AtBeginDocument{\AlsoImplementation}" >> ltxdoc.cfg
	$(LATEX) -jobname=${@:.pdf=} ${<:.sty=.dtx}
	$(MAKEINDEX) -s gind.ist ${@:.pdf=}
	$(LATEX) -jobname=${@:.pdf=} ${<:.sty=.dtx}
	$(LATEX) -jobname=${@:.pdf=} ${<:.sty=.dtx}
	rm -f ltxdoc.cfg

lstdrvrs.pdf: lstdrvrs.dtx
	echo "\PassOptionsToClass{a4paper}{article}" > ltxdoc.cfg
	$(LATEX) ${<:.sty=.dtx}
	$(MAKEINDEX) -s gind.ist lstdrvrs
	$(LATEX) ${<:.sty=.dtx}
	$(LATEX) ${<:.sty=.dtx}
	rm -f ltxdoc.cfg

## Testing targets
acm-tests:
	cd testing; make acm

algol-tests:
	cd testing; make algol

bash-tests:
	cd testing; make bash

c++11-tests:
	cd testing; make c++11

cobol-tests:
	cd testing; make cobol

fortran-tests:
	cd testing; make fortran

elisp-tests:
	cd testing; make elisp

gap-tests:
	cd testing; make gap

go-tests:
	cd testing; make go

hansl-tests:
	cd testing; make hansl

llvm-tests:
	cd testing; make llvm

lua-tests:
	cd testing; make lua

mathematica-tests:
	cd testing; make mathematica

python-tests:
	cd testing; make python

scala-tests:
	cd testing; make scala

swift-tests:
	cd testing; make swift

vbscript-tests:
	cd testing; make vbscript

xml-tests:
	cd testing; make xml

tests:
	cd testing; make all

## Clean targets
clean:
	-rm -f  *~ *.aux *.lof *.log *.lot *.tmp *.toc
	-rm -f *.idx *.ind *.glg *.glo *.gls *.ilg *.out
	-rm -f *.bbl *.blg *.brf

clean-results:
	-rm -f *.cfg *.pdf *.prf *.sty

realclean:  clean clean-results

### create packed files
tar-src:
	@$(MAKE) realclean; \
	sed -i -e "s+fileversion{[a-z0-9\.\-]*}+fileversion{$(VERSION)}+g" \
	    -e "s+filedate{[0-9/]*}+filedate{$(DATE)}+g" \
	    -e "s+date{[0-9/]*\\\\enspace+date{$(DATE)\\\\enspace+g" \
	    -e "s+Version [a-z0-9\.\-]*\\\\+Version $(VERSION)\\\\+g" \
		listings.dtx; \
	sed -i -e "s+date{[0-9/]*\\\\enspace+date{$(DATE)\\\\enspace+g" \
	    -e "s+Version [a-z0-9\.\-]*\\\\+Version $(VERSION)\\\\+g" \
	    -e "s+\[[0-9/]* [a-z0-9\.\-]* listings+[$(DATE) $(VERSION) listings+g" \
		lstdrvrs.dtx; \
	cd ..; tar $(EXsvn) -czvf $(PACKAGE)/$(TAR_SRC) $(PACKAGE)

tar-dist: $(PACKAGE_FILES)
	@$(MAKE) realclean; \
	sed -i -e "s+fileversion{[a-z0-9\.\-]*}+fileversion{$(VERSION)}+g" \
	    -e "s+filedate{[0-9/]*}+filedate{$(DATE)}+g" \
	    -e "s+date{[0-9/]*\\\\enspace+date{$(DATE)\\\\enspace+g" \
	    -e "s+Version [a-z0-9\.\-]*\\\\+Version $(VERSION)\\\\+g" \
		listings.dtx; \
	sed -i -e "s+date{[0-9/]*\\\\enspace+date{$(DATE)\\\\enspace+g" \
	    -e "s+Version [a-z0-9\.\-]*\\\\+Version $(VERSION)\\\\+g" \
	    -e "s+\[[0-9/]* [a-z0-9\.\-]* listings+[$(DATE) $(VERSION) listings+g" \
		lstdrvrs.dtx; \
	$(MAKE) listings.pdf; \
	$(MAKE) listings-devel.pdf; \
	$(MAKE) lstdrvrs.pdf; \
	tar cfvz $(PACKAGE)-$(VERSION).tgz $(DISTRIBUTION_FILES);

tagged-release:
	sed -n -e "/Version $(VERSION)/,$$$$w announcement_text.log" \
	    announcement_text.txt
	svn copy --file ./announcement_text.log \
		svn+ssh://j_hoffmann@svn.gnu.org.ua/listings/trunk \
		svn+ssh://j_hoffmann@svn.gnu.org.ua/listings/tags/$(VERSION)
	rm announcement_text.log


## Documentation target
help::
	$(info Usage:)
	$(info )
	$(info make [all]	generates listings.sty and [all] the .pdf versions)
	$(info $(empty)		(user/developer) of the documentation)
	$(info )
	$(info make <file name>)
	$(info $(empty)		creates the corresponding file denoted by <file name>)
	$(info )
	$(info make help	shows this help)
	$(info )
	$(info make tests	performs a little test suite)
	$(info )
	$(info make clean	removes all intermediate files created by a LaTeX run)
	$(info )
	$(info make clean-results)
	$(info $(empty)		removes .cfg, .sty, and .pdf files)
	$(info )
	$(info make realclean)
	$(info $(empty)		performs clean and clean-results)
	$(info )
	$(info make tar-src)
	$(info $(empty)		generates a tarred version of the current directory)
	$(info )
	$(info make tar-dist)
	$(info $(empty)		generates a distributable version of the listings)
	$(info $(empty)		package)
	$(info )
	$(info make tagged-release)
	$(info $(empty)		creates a new tagged version of the package based on)
	$(info $(empty)		the contents of listings.version and announcement_text.txt)
	@echo ""					# prevents message "nothing to do ..."

### Makefile ends here ---


==> listings/README <==
Listings package

Copyright 1996--2004 Carsten Heinz (the package)
Copyright 1996--2007 individual authors (language drivers)
Copyright 2006--2007 Brooks Moses (continued maintenance)
Copyright 2013--2020 Jobst Hoffmann (continued maintenance)

Released under the LaTeX Project Public License 1.3c or later

The `listings' package is a source code printer for LaTeX.
You can typeset stand alone files as well as listings with
an environment similar to `verbatim' as well as you can
print code snippets using a command similar to \verb'.
Many parameters control the output and if your preferred
programming language isn't already supported, you can make
your own definition.

